UniTable: Towards a Unified Framework for Table Recognition via Self-Supervised Pretraining

Tables convey factual and quantitative data with implicit conventions created by humans that are often challenging for machines to parse. Prior work on table recognition (TR) has mainly centered around complex task-specific combinations of available inputs and tools. We present UniTable, a training framework that unifies both the training paradigm and training objective of TR. Its training paradigm combines the simplicity of purely pixel-level inputs with the effectiveness and scalability empowered by self-supervised pretraining from diverse unannotated tabular images. Our framework unifies the training objectives of all three TR tasks - extracting table structure, cell content, and cell bounding box - into a unified task-agnostic training objective: language modeling. Extensive quantitative and qualitative analyses highlight UniTable's state-of-the-art (SOTA) performance on four of the largest TR datasets. UniTable's table parsing capability has surpassed both existing TR methods and general large vision-language models, e.g., GPT-4o, GPT-4-turbo with vision, and LLaVA. Our code is publicly available at https://github.com/poloclub/unitable, featuring a Jupyter Notebook that includes the complete inference pipeline, fine-tuned across multiple TR datasets, supporting all three TR tasks.

==> 901-second.tex <==
\section{Alternative}
\label{appx: second}

% another solution
% solution 1 is hard as the images are rescaled and the text are skewed. 
% learnt and shortcut that predicts <sep> without the image context
a direct ocr for all table content extraction is hard (ablations)
\textbf{Solution 1: Cell first}
For the cell first solution, the task prompt is \texttt{[cell]}, and the model is expected to predict the tokens representing the content in each cell. 
The \texttt{<sep>} token is used to separate different cells. 
The model also needs to take care of an empty cell, thus the \texttt{<empty>} token is used while an empty cell is encountered. 
While reconstructing the table, we just need to sequentially insert the text after \texttt{<td>} for a single cell or \texttt{>} for spanning cells. 
For example, the following sequence \texttt{'Low rectum', ' Male', [], ' Middle rectum', ' T3', ' T4a', ...} will be converted to \texttt{<sep> Low rectum <sep> Male <sep> <empty> <sep> Middle rectum <sep> T3 <sep> T4a <sep>}. 

2. cell bbox detection (do not punish the input sequence) (bbox)
For the bbox detection, the model performs cell localization task. 
The prompt for the task is based on the cell content. 
For example, the following sequence \texttt{[bbox] 3 cell(s) <sep> Low rectum <sep> Male <sep> <empty> <sep>} is the query to the model to perform cell localization for three consecutive cells. 
And the groundtruth output is a sequence of boxes, where each of them is represented as $[x_{min}, y_{min}, x_{max}, y_{max}]$. 
Note the empty cells do not have bbox annotations. 

==> table/appx-sota.tex <==
\begin{table}[!htbp]
\centering
\caption{Caption icdar 19 b2m wavg. F1 42.62  iou 0.6 58.10}
\begin{tabular}{lrrrrr}
\toprule
    SynthTabNet \\
\midrule
    Methods & S-\acs{teds} & \acs{map} & \acs{ap}$_{50}$ & \acs{ap}$_{75}$ \\
\midrule
    TableFormer~\cite{nassar2022tableformer} & 96.70 & - & 87.70 & - \\
    DRCC~\cite{shen2023divide} & 98.70 & - & - & - \\
    base (ours) & 98.97 & 96.43 & 98.99 & 98.79 \\
    large (ours) & 99.39 & 97.26 & 99.00 & 98.87 \\
\toprule
    PubTabNet \\
\midrule
    Methods & S-\acs{teds} & \acs{teds} & \acs{map} & \acs{ap}$_{50}$ & \acs{ap}$_{75}$ \\
\midrule
    EDD~\cite{zhong2020image} & 89.90 & 88.30 & - & 79.20 & - \\
    GTE~\cite{zheng2021global} & 93.01 & - & - & - & - \\
    TableFormer~\cite{nassar2022tableformer} & 96.75 & 93.60 & - & 82.10 & - \\
    TableMaster~\cite{ye2021pingan} & 96.04 & 96.16 & - & - & - \\
    OTSL~\cite{lysak2023optimized} & 95.50 & - & - & - & 88.00\\
    VAST~\cite{huang2023improving}  & 97.23 & 96.31 & - & 94.80 & - \\
    base (ours) & 95.63 & 94.78 & 76.84 & 97.94 & 87.27 \\
    large (ours) & 97.89 & 96.50 & 82.82 & 98.43 & 92.44 \\
\toprule
    PubTables-1M \\
\midrule
    Methods & \acs{map} & \acs{ap}$_{50}$ & \acs{ap}$_{75}$ \\
\midrule
    Faster R-CNN~\cite{smock2022pubtables} & 72.20 & 81.50 & 78.50 \\
    OTSL~\cite{lysak2023optimized} & - & - & 89.60 \\
    DETR~\cite{smock2022pubtables} & 91.20 & 97.10 & 94.80 \\
    base (ours) & 82.21 & 94.48 & 88.64 \\
    large (ours) & 87.39 & 95.68 & 93.28 \\
\toprule
    FinTabNet \\
\midrule
    Methods & S-\acs{teds} \\
\midrule
    GTE~\cite{zheng2021global} & 91.02 \\
    EDD~\cite{zhong2020image} & 90.60 \\
    OTSL~\cite{lysak2023optimized} & 95.90 \\
    TableFormer~\cite{nassar2022tableformer} & 96.80 \\
    VAST~\cite{huang2023improving} & 98.63 \\
    base (ours) & 97.19 \\
    large (ours) & 98.89 \\
\toprule
    ICDAR 2019 cTDaR \\
\midrule
\bottomrule
\end{tabular}
\label{tab:my_label}
\end{table}
